Astro2020 Decadal Science White Paper: Gravitational Wave Survey of Galactic Ultra Compact Binaries

Ultra-compact binaries (UCBs) are systems containing compact or degenerate stars with orbital periods less than one hour. Tens of millions of UCBs are predicted to exist within theGalaxy emitting gravitational waves (GWs) at mHz frequencies. Combining GW searches with electromagnetic (EM) surveys like Gaia and LSST will yield a comprehensive, multimessenger catalog of UCBs in the galaxy. Joint EM and GW observations enable measurements of masses, radii, and orbital dynamics far beyond what can be achieved by independent EM or GW studies. GW+EM surveys of UCBs in the galaxy will yield a trove of unique insights into the nature of white dwarfs, the formation of compact objects, dynamical interactions in binaries, and energetic, accretion-driven phenomena like Type Ia superonovae.

==> single_sources.tex <==
Above $\sim{}10$ mHz, UCBs are isolated from one another in frequency and have high signal-to-noise ratio making them cleanly detectable and well characterized regardless of their location in the galaxy. Thanks to their high SNR, these sources will be easily identified early in the mission (within a few weeks of observing) and well localized, thus making them excellent candidates for joint EM monitoring. These high frequency sources will also enable precision measurement of the time rate of change of the orbital period, and in some cases, the second derivative.

In general relativity (GR), the orbital evolution of two point particles, to leading post-Newtonian order (sufficient for UCBs because $v_{\rm orb}\ll c$), is completely determined by the orbital frequency and the chirp mass $\Mc\equiv \frac{(m_1 m_2)^{3/5}}{(m_1+m_2)^{1/5}}$. As discussed in Sec. \ref{sec:population}, $\Mc$ is not directly measured for typical UCBs, but is encoded in the GW amplitude $\mathcal{A}$ along with, $f$, inclination angle $\iota$, and the luminosity distance $D_L$. 

For detached UCBs evolving only due to gravitational wave emission, $\dot{f} \propto \Mc^{5/3} f^{11/3}$, thus constraining $\dot{f}$ constrains $\Mc$, and the amplitude is used to determine the distance to the source (the polarization content of the GW source helps constrain the inclination). With gravitational-wave observations alone, \checkme{20\%} of detached binaries will have $\dot{f}$ constrained to better than \checkme{10\%}. Further refinement on the distance and inclination from EM observations will enable consistency tests between the measured orbital evolution and the prediction from GR. 

Non-GR contributions to $\dot{f}$ will be monitored throughout the mission lifetime (and indefinitely for multimessenger systems) to probe astrophysical effects such as mass transfer or tidal excitation of the component objects, and as a test of alternative theories of gravity which may predict low post-Newtonian order effects such as dipole radiation~\citeme{REFS}.

%\note{Summary/transition paragraph}
